High-order flux reconstruction method for the hyperbolic formulation of the incompressible Navier-Stokes equations on unstructured grids

A high-order Flux reconstruction implementation of the hyperbolic formulation for the incompressible Navier-Stokes equation is presented. The governing equations employ Chorin's classical artificial compressibility (AC) formulation cast in hyperbolic form. Instead of splitting the second-order conservation law into two equations, one for the solution and another for the gradient, the Navier-Stokes equation is cast into a first-order hyperbolic system of equations. Including the gradients in the AC iterative process results in a significant improvement in accuracy for the pressure, velocity, and its gradients. Furthermore, this treatment allows for taking larger time-steps since the hyperbolic formulation eliminates the restriction due to diffusion. Tests using the method of manufactured solutions show that solving the conventional form of the Navier-Stokes equation lowers the order of accuracy for gradients, while the hyperbolic method is shown to provide equal orders of accuracy for both the velocity and its gradients which may be beneficial in several applications. Two- and three-dimensional benchmark tests demonstrate the superior accuracy and computational efficiency of the developed solver in comparison to the conventional method and other published works. This study shows that the developed high-order hyperbolic solver for incompressible flows is attractive due to its accuracy, stability and efficiency in solving diffusion dominated problems.

==> Eqn_INS_HINS_vert.tex <==

%% main textP
\section{Incompressible Navier-Stokes Equations}
Consider the incompressible Navier-Stokes equations in artificial compressibility form \cite{CHORIN196712}:

\begin{equation} \label{ins_eqns}
    \begin{split}
        &{\partial p \over \partial \tau}  + \nabla \cdot ( \zeta \textbf{v} ) = 0 \\
        &{\partial \textbf{v} \over \partial \tau}  + \nabla \cdot (\textbf{v}\otimes  \textbf{v} + p - \nu \nabla \textbf{v}) =0
        \end{split}
\end{equation}
where \textbf{v} is the velocity vector, $p$ is the pressure, $\nu$ is the kinematic viscosity, $\zeta$ is the the artificial compressiblity relaxation factor and $\tau$ is the psuedo-time used to drive the solution to steady state.

The hyperbolic formulation of the equation is obtained by inserting $\textbf{g} = \nabla\textbf{v}$ in 
\cref{ins_eqns} and introducing an additional equation for \textbf{g}
\begin{equation} \label{hins_eqns}
    \begin{split}
        &{\partial p \over \partial \tau}  + \nabla \cdot ( \zeta \textbf{v} ) = 0 \\
        &{\partial \textbf{v} \over \partial \tau}  + \nabla \cdot (\textbf{v}\otimes  \textbf{v} + p\textbf{I} - \nu \textbf{g}) =0 \\
        & {\partial \textbf{g} \over \partial \tau} = {1 \over T_r}(\nabla\textbf{v}  - \textbf{g} )
    \end{split}
\end{equation}
where $T_r$ is the relaxation time given
\begin{equation}
   T_r = L^2/\nu 
\end{equation}
The length scale $L$ is defiend as $L = 1/{2\pi}$. At psuedo-time steady-state $\textbf{g} = \nabla\textbf{v}$ and the incompressible Navier-Stokes equations are recovered. 
More details regarding the hyperbolic formulation is cited in the previous section and thus not mentioned here.

In three dimensions, the conservative variables for the hyperbolic incompressible Navier-Stokes (HINS) equations are
\begin{equation}
    u_\alpha = \begin{Bmatrix}
        p\\
        v_x\\
        v_y\\
        v_z\\
        g_{xx}\\
        g_{xy}\\
        g_{xz}\\
        g_{yx}\\
        g_{yy}\\
        g_{yz}\\
        g_{zx}\\
        g_{zy}\\
        g_{zz}\\
        \end{Bmatrix}
\end{equation}
where $v_x,~ v_y,~ v_z$ are the velocity components, $g_{ij}$ is the gradient of the $i^{th}$ velocity component in the $j^{th}$ direction. The fluxes are given are 

\begin{equation}
    \textbf{f}_\alpha = 
    \begin{Bmatrix}
       f^e_{\alpha x} - f^v_{\alpha x}\\
       f^e_{\alpha y} - f^v_{\alpha y}\\
       f^e_{\alpha z} - f^v_{\alpha z}
    \end{Bmatrix}
\end{equation}
where
\begin{equation}
    \textbf{f}^e_{\alpha x} = 
    \begin{Bmatrix}
       \zeta v_x\\
           v_x^2 + p\\
           v_x v_y\\
           v_x v_z\\
           -{1 \over T_r}v_x\\
           0\\
           0\\
           -{1 \over T_r}v_y\\
           0\\
           0\\
           -{1 \over T_r}v_z\\
           0\\
           0\\
    \end{Bmatrix}, \qquad
    \textbf{f}^e_{\alpha y} = 
    \begin{Bmatrix}
            \zeta v_y\\
            v_y v_x\\
           v_y^2 + p\\
           v_z v_x\\
           0\\
           -{1 \over T_r}v_x\\
           0\\
           0\\
           -{1 \over T_r}v_y\\
           0\\
           0\\
           -{1 \over T_r}v_z\\
           0\\
    \end{Bmatrix}, \qquad
    \textbf{f}^e_{\alpha z} = 
    \begin{Bmatrix}
            \zeta v_z\\
            v_z v_x\\
            v_z v_y\\
           v_z^2 + p\\        
           0\\
           0\\
           -{1 \over T_r}v_x\\
           0\\
           0\\
           -{1 \over T_r}v_y\\
           0\\
           0\\
           -{1 \over T_r}v_z\\
    \end{Bmatrix}
\end{equation} 


\begin{equation}
    \textbf{f}^v_{\alpha x} = 
    \begin{Bmatrix}
       0\\
       \nu  g_{xx}\\
       \nu  g_{yx}\\
       \nu  g_{zx}\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
    \end{Bmatrix}, \qquad
    \textbf{f}^v_{\alpha y} = 
    \begin{Bmatrix}
        0\\
        \nu g_{xy}\\
        \nu  g_{yy}\\
        \nu  g_{zy}\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
    \end{Bmatrix}, \qquad
    \textbf{f}^v_{\alpha z} = 
    \begin{Bmatrix}
        0\\
        \nu  g_{xz}\\
        \nu  g_{yz}\\
        \nu  g_{zz}\\      
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
           0\\
    \end{Bmatrix}
\end{equation} 
It should be noted that $\textbf{f}_\alpha $ is no longer dependent on $\nabla u_\alpha$ but it is simply $\textbf{f}_\alpha = \textbf{f}_\alpha(u_\alpha) $.


The source term is defined by 
\begin{equation}
    S = {1 \over T_r}\begin{Bmatrix}
        0\\
        0\\
        0\\
        0\\
        -g_{xx}\\
        -g_{xy}\\
        -g_{xz}\\
        -g_{yx}\\
        -g_{yy}\\
        -g_{yz}\\
        -g_{zx}\\
        -g_{zy}\\
        -g_{zz}\\
        \end{Bmatrix}
\end{equation}

==> MMS_SandiaCase.tex <==

% \documentclass[preprint,12pt]{elsarticle}


% \usepackage{amssymb}

% \usepackage{lineno}

% \usepackage{natbib}


% \journal{Journal Name}

% \begin{document}

% \begin{frontmatter}


%     \title{HINS for PyFR}


%     \author{Mohamed Kamra \& Jabir AlSalami \& Changhong Hu}

%     \address{Fukuoka, Japan}

%     \begin{abstract}
%         %% Text of abstract
%         Suspendisse potenti. Suspendisse quis sem elit, et mattis nisl. Phasellus consequat erat eu velit rhoncus non pharetra neque auctor. Phasellus eu lacus quam. Ut ipsum dolor, euismod aliquam congue sed, lobortis et orci. Mauris eget velit id arcu ultricies auctor in eget dolor. Pellentesque suscipit adipiscing sem, imperdiet laoreet dolor elementum ut. Mauris condimentum est sed velit lacinia placerat. Vestibulum ante ipsum primis in faucibus orci luctus et ultrices posuere cubilia Curae; Nullam diam metus, pharetra vitae euismod sed, placerat ultrices eros. Aliquam tincidunt dapibus venenatis. In interdum tellus nec justo accumsan aliquam. Nulla sit amet massa augue.
%     \end{abstract}

%     \begin{keyword}
%         Science \sep Publication \sep Complicated


%     \end{keyword}

% \end{frontmatter}

% \linenumbers




%% main text
\section{MMS Sandia Case}
\label{S:1}

In this section, we apply the method of manufactured solutions(MMS) to the incompressible Navier-Stokes equations.
The method is applied to both the conventional and hyperbolic formulations of the equations.
We use the MMS procedure outlined by \citeauthor{salari2000code} \cite{salari2000code}.
The steady manufactured solution provided in the report for incompressible laminar flow is used while setting the constants $ u_0 = v_0 = P_0 = 1$ and $ \varepsilon  = 0$.
\begin{equation}\label{mms_u}
    u(x,y) = u_0  sin(x^2 + y^2)  + \varepsilon
\end{equation}
\begin{equation}\label{mms_v}
    v(x,y) = v_0 cos(x^2 + y^2) + \varepsilon
\end{equation}
\begin{equation}\label{mms_p}
    p(x,y) = P_0  sin(x^2 + y^2) + 2.0
\end{equation}
%% TODO: Maybe revise and use the source term included in the report
The source term are generated by plugging the manufactured in the governing equation and simplifying the resulting expression using SymPy. Dirichlet boundary conditions were used on all boundaries. Similar to the article, the simulation was conducted for a kinematic viscosity $\nu$ =0.5, artificial compressibility constant $\beta = 40 $, and a convergence tolerance of $10^{-12}$.
Four uniform quadrilateral grids, 6x5, 11x9, 21x17, and 41x33, with a uniform mesh refinement ratio of two were used to compute the order of accuracy of the solution variable Q=($p$,$u$,$v$) and their gradients $\nabla Q$ . The grids are denoted by $\Omega^i$ with $\Omega^1$ on the coarsest grid to $\Omega^4$ on the finest grid. The number of degrees of freedom is denoted by $N_{DOF}$ which represents the total number of solution in $\Omega^i$. The error with manufactured solution is quantified using  $L^2$-norm computed by
\begin{equation}
    \| \epsilon \|  =  \sqrt{ \frac{\sum_{k = 1}^{N_{DOF}}  \epsilon^2 }{N_{DOF}}}
\end{equation}
where $\epsilon = \widetilde{Q} (x,y) - Q(x,y)$ and $\widetilde{Q} (x,y)$  is the manufactured solution and $Q(x,y)$ is the solution obtained numerically evaluated at the solution points to avoid interpolation errors contaminating the results.
The order of accuracy $\mathcal{P}$  is then evaluated using
\begin{equation}
    \mathcal{P} = \frac{\log{\left[\frac{\| \epsilon \|(\Omega^i)}{\| \epsilon \|(\Omega^{i+1})} \right] }} {\log{\left[\frac{h(\Omega^i)}{h(\Omega^{i+1})} \right] }}
\end{equation}
where $ h(\Omega^i) = 1/\sqrt{N_{DOF}}$ for $\Omega^i \subset \mathbb{R} ^2$. The value of relaxation time ($T_r$) chosen for HINS-FR is 190. The choice is based on a series of numerical experiments which will presented in detail in the following section. 


\begin{table}[htbp]
    \caption{Method of manufactured solutions problem, observed order of accuracy for HINS-FR system and INS-FR original system for p = 3}
    \label{<label>}
    \centering\begin{tabular}{lrlrlrl}
        \hline
                   & \multicolumn{2}{c}{$u$} & \multicolumn{2}{c}{$\partial u \over \partial x$} & \multicolumn{2}{c}{$\partial u \over \partial y$}                              \\
        Grid       & $L^2$-norm              & order                     & $L^2$-norm                & order & $L^2$-norm & order \\
        \hline \\
        (a) HINS-FR \\
        $\Omega^1$ & 1.15E-06 & -    & 2.86E-06 & -    & 5.14E-06 & -    \\
        $\Omega^2$ & 6.58E-08 & 4.12 & 1.70E-07 & 4.08 & 2.99E-07 & 4.10 \\
        $\Omega^3$ & 3.99E-09 & 4.05 & 1.06E-08 & 4.00 & 1.81E-08 & 4.05 \\
        $\Omega^4$ & 2.46E-10 & 4.02 & 6.70E-10 & 3.99 & 1.11E-09 & 4.00 \\
        \\
        (b) INS-FR \\ 
        $\Omega^1$ & 1.62E-06                & -                         & 1.60E-04                  & -     & 1.94E-04   & -     \\
        $\Omega^2$ & 1.04E-07                & 3.96                      & 2.01E-05                  & 3.00  & 2.46E-05   & 2.98  \\
        $\Omega^3$ & 6.84E-09                & 3.93                      & 2.51E-06                  & 3.00  & 3.10E-06   & 2.99  \\
        $\Omega^4$ & 4.40E-10                & 3.96                      & 3.15E-07                  & 3.00  & 3.89E-07   & 2.99  \\
        \\

    \end{tabular}


\end{table}

\subsection{Effect of $T_r$ on accuracy}
The choice of the relaxation time ($T_r$) plays an important role not only in the convergence behavior of HINS-FR system but also the accuracy and order of accuracy of the numerical solution as highlighted here.

While there are several formulas that estimate the best choice for $T_r$, we found the optimum value which provides lowest error and best convergence rate to be quite far from the values provided by such formulas. For problems where the exact solution is known, a simple trial and error would  suffice. The accuracy of solution would not suffer much as long as the used value within $20\%$ of what it should be.
We conducted a several of numerical experiments to identify the sensitivity of the optimum $T_r$ value to the problem parameters.
First we start the problems parameters that affect the choice of $T_r$ which the artificial compressibility constant ($\beta$ ), the order of solution polynomial ($q$)), mesh resolution ($h$). On the other hand, the kinematic viscosity ($\nu$), problem scale/reference length ($L_r$) , and reference velocity ($U_r$) were found to strongly affect the optimum $T_r$. While at a first glance, these parameters constitute the Reynolds number we already confirmed that for the same Reynolds number different combinations of ($U_r,~L_r, and~\nu $) do not give the same optimum ($T_r$) value.




% % \begin{itemize}
% %     \item Bullet point one
% %     \item Bullet point two
% % \end{itemize}

% % \begin{enumerate}
% %     \item Numbered list item one
% %     \item Numbered list item two
% % \end{enumerate}

% % \subsection{Subsection One}

% % Quisque elit ipsum, porttitor et imperdiet in, facilisis ac diam. Nunc facilisis interdum felis eget tincidunt. In condimentum fermentum leo, non consequat leo imperdiet pharetra. Fusce ac massa ipsum, vel convallis diam. Quisque eget turpis felis. Curabitur posuere, risus eu placerat porttitor, magna metus mollis ipsum, eu volutpat nisl erat ac justo. Nullam semper, mi at iaculis viverra, nunc velit iaculis nunc, eu tempor ligula eros in nulla. Aenean dapibus eleifend convallis. Cras ut libero tellus. Integer mollis eros eget risus malesuada fringilla mattis leo facilisis. Etiam interdum turpis eget odio ultricies sed convallis magna accumsan. Morbi in leo a mauris sollicitudin molestie at non nisl.

% % \begin{table}[h]
% %     \centering
% %     \begin{tabular}{l l l}
% %         \hline
% %         \textbf{Treatments} & \textbf{Response 1} & \textbf{Response 2} \\
% %         \hline
% %         Treatment 1         & 0.0003262           & 0.562               \\
% %         Treatment 2         & 0.0015681           & 0.910               \\
% %         Treatment 3         & 0.0009271           & 0.296               \\
% %         \hline
% %     \end{tabular}
% %     \caption{Table caption}
% % \end{table}

% % \subsection{Subsection Two}

% % Donec eget ligula venenatis est posuere eleifend in sit amet diam. Vestibulum sollicitudin mauris ac augue blandit ultricies. Nulla facilisi. Etiam ut turpis nunc. Praesent leo orci, tincidunt vitae feugiat eu, feugiat a massa. Duis mauris ipsum, tempor vel condimentum nec, suscipit non mi. Fusce quis urna dictum felis posuere sagittis ac sit amet erat. In in ultrices lectus. Nulla vitae ipsum lectus, a gravida erat. Etiam quam nisl, blandit ut porta in, accumsan a nibh. Phasellus sodales euismod dolor sit amet elementum. Phasellus varius placerat erat, nec gravida libero pellentesque id. Fusce nisi ante, euismod nec cursus at, suscipit a enim. Nulla facilisi.

% % % \begin{figure}[h]
% % % \centering\includegraphics[width=0.4\linewidth]{placeholder}
% % % \caption{Figure caption}
% % % \end{figure}

% % Integer risus dui, condimentum et gravida vitae, adipiscing et enim. Aliquam erat volutpat. Pellentesque diam sapien, egestas eget gravida ut, tempor eu nulla. Vestibulum mollis pretium lacus eget venenatis. Fusce gravida nisl quis est molestie eu luctus ipsum pretium. Maecenas non eros lorem, vel adipiscing odio. Etiam dolor risus, mattis in pellentesque id, pellentesque eu nibh. Mauris nec ante at orci ultricies placerat ac non massa. Aenean imperdiet, ante eu sollicitudin vestibulum, dolor felis dapibus arcu, sit amet fermentum urna nibh sit amet mauris. Suspendisse adipiscing mollis dolor quis lobortis.

% % \begin{equation}
% %     \label{eq:emc}
% %     e = mc^2
% % \end{equation}

% % \section{The Second Section}
% % \label{S:2}

% % Reference to Section \ref{S:1}. Etiam congue sollicitudin diam non porttitor. Etiam turpis nulla, auctor a pretium non, luctus quis ipsum. Fusce pretium gravida libero non accumsan. Donec eget augue ut nulla placerat hendrerit ac ut mi. Phasellus euismod ornare mollis. Proin tempus fringilla ultricies. Donec pretium feugiat libero quis convallis. Nam interdum ante sed magna congue eu semper tellus sagittis. Curabitur eu augue elit.

% % Aenean eleifend purus et massa consequat facilisis. Etiam volutpat placerat dignissim. Ut nec nibh nulla. Aliquam erat volutpat. Nam at massa velit, eu malesuada augue. Maecenas sit amet nunc mauris. Maecenas eu ligula quis turpis molestie elementum nec at est. Sed adipiscing neque ac sapien viverra sit amet vestibulum arcu rhoncus.

% % Vivamus pharetra nibh in orci euismod congue. Pellentesque habitant morbi tristique senectus et netus et malesuada fames ac turpis egestas. Quisque lacus diam, congue vel laoreet id, iaculis eu sapien. In id risus ac leo pellentesque pellentesque et in dui. Etiam tincidunt quam ut ante vestibulum ultricies. Nam at rutrum lectus. Aenean non justo tortor, nec mattis justo. Aliquam erat volutpat. Nullam ac viverra augue. In tempus venenatis nibh quis semper. Maecenas ac nisl eu ligula dictum lobortis. Sed lacus ante, tempor eu dictum eu, accumsan in velit. Integer accumsan convallis porttitor. Maecenas pretium tincidunt metus sit amet gravida. Maecenas pretium blandit felis, ac interdum ante semper sed.

% % In auctor ultrices elit, vel feugiat ligula aliquam sed. Curabitur aliquam elit sed dui rhoncus consectetur. Cras elit ipsum, lobortis a tempor at, viverra vitae mi. Cras sed urna sed eros bibendum faucibus. Morbi vel leo orci, vel faucibus orci. Vivamus urna nisl, sodales vitae posuere in, tempus vel tellus. Donec magna est, luctus non commodo sit amet, placerat et enim.



% %% References with bibTeX database:

% \bibliographystyle{model1-num-names}
% \bibliography{references.bib}




% \end{document}



==> Method_FluxReconstruction_Steps.tex <==
The steps of solving equations \ref{maintranseq} and \ref{maintranseq2} are as follows:

\paragraph{Step 1:}
In order to compute gradients (Eq. \ref{maintranseq2}), the  continuous solution across element boundaries is first reconstructed. The discontinuous solution in the \textit{n}th element at the \textit{i}th flux point $u_{ni}^{f}$ is approximated by interpolating from the discontinuous solution at solution points $u_{nj}^{u}$ using the polynomial nodal basis

\begin{equation} \label{extrapolateSoln}
	u_{ni}^{f} = \sum_{j=1}^{N_{n}^{f}}u_{nj}^{u} \mathit{l}_{nj}(\tilde{\mathbf{x}}_{ni}^{f})
\end{equation}

\paragraph{Step 2:}
By adopting the Local Discontinuous Galerkin approach, the common solution at flux points is then computed 

\begin{equation}
	\mathfrak{C}(u^{f}_{ni}) =\mathfrak{C}(u^{f}_{n^\prime i^\prime}) = (\frac{1}{2}- \beta)u^{f}_{ni}+ (\frac{1}{2}+ \beta) u^{f}_{n^\prime i^\prime}
\end{equation}

where $n^\prime i^\prime$ denote the coinciding flux point of a neighboring element, and the  parameter  $\beta = \pm \frac{1}{2}$

\paragraph{Step 3:}
The gradient of the continuous solution at solution points is computed using

\begin{equation} \label{continuousGrad}
	\tilde{\mathbf{q}}_{ni}^{u} = \sum_{j=1}^{N_n^{f}}\left[ \widehat{\tilde{\mathbf{n}}}_{nj} \cdot \tilde{\nabla} \cdot \mathbf{g}_{nj}(\mathbf{\tilde{x}}_{ni}^{u}) \left(\mathfrak{C}(u^{f}_{nj}) - u^{f}_{nj} \right) \right] + \sum_{j=1}^{N_n^{u}} \left[ u^{u}_{nj} \tilde{\nabla} \mathit{l}_{nj}^{u}(\mathbf{\tilde{x}}_{ni}^{u})\right]
\end{equation}

where $\tilde{\mathbf{n}}$ is the normalized and transformed outward-pointing normal vector at the flux points, and $\mathbf{g}_{nj}(\mathbf{x}^{u})$ is the vector correction function associated with each flux point, which is used to ensure gradient continuity across element interfaces and is required to satisfy

\begin{equation}
\widehat{\tilde{\mathbf{n}}}_{ni} \cdot \mathbf{g}_{nj}(\mathbf{x}_{ni}^{f}) = \delta_{ij}
\end{equation}

The transformed solution's gradient is mapped back to physical space using $\mathbf{q}_{ni}^{u} = \mathbf{J}^{-T} \tilde{\mathbf{q}}_{ni}^{u}$, and then evaluated at flux points, using the same procedure in \ref{extrapolateSoln}

\begin{equation} \label{extrapolateGrad}
\mathbf{q}_{ni}^{f} = \sum_{j=0}^{N_{n}^{f}}\mathbf{q}_{nj}^{u} \mathit{l}_{nj}(\tilde{\mathbf{x}}_{ni}^{f})
\end{equation}

\paragraph{Step 4:}

Using the transformed gradient found in the previous steps, the flux is evaluated at solution points in transformed space according to

\begin{equation}
\tilde{\mathbf{f}}_{ni}^{u} =\mathcal{J}_{ni}\mathbf{J}^{-1}_{ni} \mathbf{f}(u_{ni}^{u}, \mathbf{q}_{ni}^{u}).
\end{equation}

Using this, the normal transformed flux at flux points is computed in a similar manner to Eqs. \ref{extrapolateSoln} and \ref{extrapolateGrad}

\begin{equation}\label{normalTransFlux}
\tilde{f}_{ni}^{f\perp} = \sum_{j=0}^{N_{n}^{f}} \widehat{\tilde{\mathbf{n}}} \cdot \tilde{\mathbf{f}}_{ni}^{u} \mathit{l}_{nj}(\tilde{\mathbf{x}}_{ni}^{f})
\end{equation}

\paragraph{Step 5:} 

In order to find the continuous flux,  common normal flux at flux points is computed using

\begin{equation} \label{commonFlux}
\mathfrak{F}(f_{ni}^{f\perp}) = -\mathfrak{F}(f_{n^\prime i^\prime}^{f\perp}) = 	\mathfrak{F}^{(inv)}(f_{ni}^{f(inv)})-\mathfrak{F}^{(vis)}(f_{ni}^{f(vis)})
\end{equation}

Note that unlike the \textit{discontinuous normal flux} found in Eq. \ref{normalTransFlux}, the \textit{common normal flux} is found using quantities extrapolated from solution points from both sides of the interface, i.e. $ u_{in}^{f},u_{i^\prime n^\prime}^{f}, \mathbf{q}_{in}^{f}$ and $\mathbf{q} _{i^\prime n^\prime}^{f}$.  The inviscid part is simply the average of inviscid normal fluxes

\begin{equation}\label{inviscidFlux}
\mathfrak{F}^{(inv)}(f_{ni}^{f(inv)})= \widehat{\mathbf{n}}_{ni} \cdot \left[ \frac{f_{ni}^{f(inv)}+f_{n^\prime i^\prime}^{f(inv)}}{2} \right]
\end{equation}

and the viscous part is found using the LDG approach

\begin{equation}\label{viscousFlux}
\mathfrak{F}^{(vis)}(f_{ni}^{f(vis)})= \widehat{\mathbf{n}} \cdot \left[\left(\frac{1}{2}+\beta\right) \mathbf{f}_{ni}^{f} + \left(\frac{1}{2}-\beta\right) \mathbf{f}_{n^\prime i^\prime}^{f} \right] + \tau(u_{ni}^{f}-u_{n^\prime i^\prime}^{f}).
\end{equation}

Common normal fluxes are then scaled and transformed to standard element space to prepare for the final step.

\paragraph{Step 6:}

The divergence of the continuous flux is obtained via a procedure that is analogous to Eq. \ref{continuousGrad}

\begin{equation} \label{continuousDivFlux}
\tilde{\nabla} \cdot \mathbf{\tilde{f}}_{ni}^{u} = \sum_{j=0}^{N_n^{f}}\left[ \tilde{\nabla} \cdot \mathbf{\tilde{g}}_{nj}(\mathbf{x}_{ni}^{u}) \left(\mathfrak{F}(\tilde{f}_{nj}^{f\perp}) - \tilde{f}^{(f \perp)}_{nj} \right) \right] + \sum_{j=0}^{N_n^{u}} \left[ \mathbf{\tilde{f}}^{u}_{nj} \cdot \tilde{\nabla} \mathit{l}_{nj}^{u}(\mathbf{\tilde{x}}_{ni}^{u})\right]
\end{equation}

the divergence of the flux at each solution point is then marched in time using a suitable time-stepping scheme 
\begin{equation}
	\frac{\partial u^{u}_{ni}}{\partial t} = - \mathcal{J}^{-1}_{ni} \tilde{\nabla} \cdot \tilde{\mathbf{f}}_{ni}^{u}
\end{equation}

==> pyFR_Impl.tex <==
\subsection{Implementation}
% The developed hyperbolic incompressible flow solver, hereafter referred to as HINS-FR, is implemented in the framework of the open-source code PyFR.  
% PyFR is a cross-platform framework for solving advection-diffusion equations using the FR approach. 
% This framework allows the generation of platform portable code using a single implementation via Python and MAKO templates. 
% For more details on the PyFR open-source software, the reader is referred to the following works\cite{witherden2015development_FR,WITHERDEN2015173_FR,LOPPI2018193_FR,LOPPI2019108913_FR}. 

% The developed HINS-FR is implemented as a separate module in the directory pyfr/solvers/ with the designation HACNavierStokes as the class name. 
% Following the ACSystem class, the HACNavierStokes class inherits a pipeline of kernel calls to do FR discretization for advection equation unlike ACNavierStokes,  which inherits the advection-diffusion system.  
% Therefore, all building blocks and macro functions related to viscous fluxes, such as LDG flux operation and LDG boundary conditions, are considered unnecessary and thus discarded. 
% The Riemann solvers are also modified to include the additional wave-speed introduced by the hyperbolic formulation, $c_v = \sqrt{\nu/T_r} $.  


For the HACNavierStokes solver, the boundary conditions are implemented via ghost states as required by the Riemann solver. Unlike the ACSystem solvers, only one ghost state is needed per boundary condition since LDG related boundary conditions are no longer present. A summary of the boundary conditions currently implemented in the HACNavierStokes solver and the corresponding ghost states is presented in \Cref{table:pyfr_hac_bcs}. 

% In this work, the conventional AC system existing in PyFR is denoted INS-FR while the developed hyperbolic AC method is denoted HINS-FR. 
% \begin{table}[htbp!] 
%     \begin{tabular}{@{}lllll@{}}
%     \toprule
%     \begin{tabular}[c]{@{}l@{}}Boundary\\ Name\end{tabular} & No Slip Wall & Slip Wall & Velocity Inlet & Pressure Outlet \\ \midrule
%     $p$      & $p_L$           & $p_L$                & $p_L$   & $p^b$    \\
%     $v_x$    & $2v_x^w-v_{xL}$ & $v_{xL}-2n_x v_{nL}$ & $v_x^b$ & $v_{xL}$ \\
%     $v_y$    & $2v_x^w-v_{xL}$ & $v_{yL}-2n_y v_{nL}$ & $v_y^b$ & $v_{yL}$ \\
%     $v_z$    & $2v_x^w-v_{xL}$ & $v_{zL}-2n_z v_{nL}$ & $v_z^b$ & $v_{zL}$ \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\
%     $g_{xx}$ & $g_{xxL}$       & 0                    & 0       & 0        \\ \bottomrule
%     \end{tabular}
%     \end{table}

\begin{table}[htbp!] 
    \centering
    \caption{Summary of ghost states for the boundary conditions implemented in HINS-FR solver (HACNavierStokes) in PyFR. 
    % $g_{ij}$ is the velocity gradient tensor for the $i^{th}$ velocity in the $j^{th}$ direction.\\
     The superscript $b$ and subscript $L$ denote the desired boundary value and left state respectively}
    \label{table:pyfr_hac_bcs}
    \begin{tabular}{@{}cccc@{}}
        \toprule
                 & \multicolumn{3}{c}{Boundary Condition Type}    \\ \cmidrule(l){2-4}
        \begin{tabular}[c]{@{}c@{}}State \\ Variable\end{tabular} & No Slip Wall & Velocity Inlet & Pressure Outlet \\ \midrule
        $p$      & $p_L$           & $p_L$   & $p^b$    \\
        $v_x$    & $2v_x^b-v_{xL}$ & $v_x^b$ & $v_{xL}$ \\
        $v_y$    & $2v_y^b-v_{yL}$ & $v_y^b$ & $v_{yL}$ \\
        $v_z$    & $2v_z^b-v_{zL}$ & $v_z^b$ & $v_{zL}$ \\
        $g_{ij}$ & $g_{ijL}$       & 0       & 0        \\ \bottomrule
        \end{tabular}
    \end{table}

% \begin{table}[htbp!] 
%     \centering
%     \caption{Summary of ghost states for the boundary conditions implmeneted in HINS-FR solver (HACNavierStokes) in PyFR}
%     \label{table:pyfr_hac_bcs}
%     \begin{tabular}{@{}cccc@{}}
%         \toprule
%                  & \multicolumn{3}{c}{Boundary Condition Type}    \\ \cmidrule(l){2-4}
%         \begin{tabular}[c]{@{}c@{}}State \\ Variable\end{tabular} & No Slip Wall & Velocity Inlet & Pressure Outlet \\ \midrule
%         $p$      & $p_L$           & $p_L$   & $p^b$    \\
%         $v_x$    & $2v_x^w-v_{xL}$ & $v_x^b$ & $v_{xL}$ \\
%         $v_y$    & $2v_y^w-v_{yL}$ & $v_y^b$ & $v_{yL}$ \\
%         $v_z$    & $2v_z^w-v_{zL}$ & $v_z^b$ & $v_{zL}$ \\
%         $g_{xx}$ & $g_{xxL}$       & 0       & 0        \\
%         $g_{xy}$ & $g_{xyL}$       & 0       & 0        \\
%         $g_{xz}$ & $g_{xzL}$       & 0       & 0        \\
%         $g_{yx}$ & $g_{yxL}$       & 0       & 0        \\
%         $g_{yy}$ & $g_{yyL}$       & 0       & 0        \\
%         $g_{yz}$ & $g_{yzL}$       & 0       & 0        \\
%         $g_{zx}$ & $g_{zxL}$       & 0       & 0        \\
%         $g_{zy}$ & $g_{zyL}$       & 0       & 0        \\
%         $g_{zz}$ & $g_{zzL}$       & 0       & 0        \\ \bottomrule
%         \end{tabular}
%     \end{table}
